Using Machine Learning to Select High-Quality Measurements

We describe the use of machine learning algorithms to select high-quality measurements for the Mu2e experiment. This technique is important for experiments with backgrounds that arise due to measurement errors. The algorithms use multiple pieces of ancillary information that are sensitive to measurement quality to separate high-quality and low-quality measurements.

==> discussion.tex <==
\section{?Discussion?}
\label{sec:discussion}
As with all machine learning methods, one must worry about inadvertantly introducing biases based on the training sample that was used.

A common worry is ``overtraining'' where a statistical fluctuation in the training sample is picked up by the ANN and interpreted as a real effect. This can be checked by using different training and test samples, and TMVA offer plots to check the ANN is not overtrained.

In our example, we trained on high-energy electrons coming from a stopping target and so we must not over apply this specific training to tracks not from this.

Understanding the systematic uncertainties introduced will also be important. We must make sure that the underlying input variable distributions are the same between real data and simulated data.

%% \begin{itemize}
%% \item{discuss overtraining?}
%% \item{determining usefulness of input variables?}
%% \item{calculating efficiency of cut?}
%% \item{evaluating systematic uncertainties?}
%% \item{possible physics biases?}
%% \end{itemize}


==> systematics.tex <==
\section{Systematic Uncertainties}
\label{sec:systematics}

\subsection{Particle Selection}
We also use graphical cuts at 2$\sigma$?

\subsection{Unfolding}
Modified the various unfolding parameters.

\subsection{Particle Composition}
For the active target analysis, we have large uncertainties on the particle composition. For the recoil and escape corrections we reevaluate with fewer protons and with more protons.

